Parameter-Efficient Prompt Tuning Makes Generalized and Calibrated Neural Text Retrievers

Prompt tuning attempts to update few task-specific parameters in pre-trained models. It has achieved comparable performance to fine-tuning of the full parameter set on both language understanding and generation tasks. In this work, we study the problem of prompt tuning for neural text retrievers. We introduce parameter-efficient prompt tuning for text retrieval across in-domain, cross-domain, and cross-topic settings. Through an extensive analysis, we show that the strategy can mitigate the two issues -- parameter-inefficiency and weak generalizability -- faced by fine-tuning based retrieval methods. Notably, it can significantly improve the out-of-domain zero-shot generalization of the retrieval models. By updating only 0.1% of the model parameters, the prompt tuning strategy can help retrieval models achieve better generalization performance than traditional methods in which all parameters are updated. Finally, to facilitate research on retrievers' cross-topic generalizability, we curate and release an academic retrieval dataset with 18K query-results pairs in 87 topics, making it the largest topic-specific one to date.

==> 5_exp.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{OAG-QA's statistics and examples.} Upper: \textmd{Comparison between existing scientific retrieval dataset (SciFact~\cite{wadden2020fact}, SCIDOCS~\cite{cohan2020specter}, TREC-COVID~\cite{voorhees2021trec}) and OAG-QA.} Lower: \textmd{Some examples of disciplines, topics, and query-paper pairs in OAG-QA.}}
    \small
    \renewcommand\tabcolsep{1pt}
    \input{tables/sci-dataset}
    \newline
    \vspace*{2mm}
    \newline
    \renewcommand\tabcolsep{1pt}
    \input{tables/oagqa-examples}
    \label{tab:oag-qa-stats}
\end{table}

\subsection{OAG-QA: A Fine-grained Cross-topic Scientific Literature Retrieval Dataset}
In response to the cross-topic generalization challenge, we present a novel fine-grained topic-specific passage retrieval dataset OAG-QA by collecting high-quality questions and answers from Online Question-and-Answers (Q\&A) forums, such as Quora and Stack Exchange. These forums offer people chances to ask questions and receive answers from other expert users, potentially with reference to academic papers. These references can be consequently aligned to paper entities with rich meta-information (e.g. abstract, field-of-study (FOS)) in the Open Academic Graph (OAG)~\cite{zhang2019oag}.


We collect questions from two influential websites: Stack Exchange\footnote{https://stackexchange.com/sites} in English, and Zhihu\footnote{https://www.zhihu.com} in Chinese. On top of the collected pairs of questions and paper titles, we align them to OAG~\cite{zhang2019oag,wang2020microsoft,tang2008arnetminer} paper ids via public API\footnote{https://www.aminer.cn/restful\_service}. In terms of topics, disciplines from Stack Exchange and tags from Zhihu naturally serve as fine-grained topics attached to collected questions. \hide{For most collected topics, we directly link them to OAG field-of-study via string matching; few rest of them are aligned and deduplicated manually.}

\hide{
\vpara{Q\&A collecting.}
We collect questions from two influential websites: Stack Exchange\footnote{https://stackexchange.com/sites} in English, and Zhihu\footnote{https://www.zhihu.com} in Chinese. Stack Exchange consists of a series of forums for specific disciplines, such as data science, biology and mathematics; Zhihu questions are not clearly divided by several disciplines, but each question is marked by fine-grained tags. We focus on five types of reference URLs from the answer context: \emph{arxiv.org}, \emph{dl.acm.org}, \emph{doi.org}, \emph{researchgate.net}, \emph{www.nature.com}, retrieve paper titles via visiting the URLs. For questions in Chinese, we translate them to English using commercial machine translation API with human proofread. 


\vpara{Paper\&Topic alignment.}
On top of the collected pairs of questions and paper titles, we align them to OAG~\cite{zhang2019oag,wang2020microsoft,tang2008arnetminer} paper ids via public API\footnote{https://www.aminer.cn/restful\_service}, which is the largest publicly available academic graphs consisting of over 370M authors, 380M papers, 120K venues, 80K academic institutes, 600K fields of study and 20B relationships between them. It also covers a wide range of text resources, including over 6 million paper full-text and 110 million paper abstracts intensely associated with graph structure.

In terms of topics, disciplines from Stack Exchange and tags from Zhihu naturally serve as fine-grained topics attached to collected questions. For most collected topics, we directly link them to OAG field-of-study via string matching; few rest of them are aligned and deduplicated manually.}

Consequently, we present OAG-QA (Cf. Table~\ref{tab:oag-qa-stats}) which consists of 17,948 unique queries from 22 scientific disciplines and 87 fine-grained topics. Given each topic, we sample 10,000 candidate papers including the groundtruth, and take their titles and abstracts as the corpus.

\hide{
\subsubsection{Stack Exchange}
Stack Exchange consists of a series of forums for specific disciplines, such as data science, biology and mathematics. We select 11 sites and use the questions from them as our data source. For each post, we retrieve all of its first-level answers, i.e. we ignore the comments inside the answer because they are less direct to the question than the first-level answers \cite{lamurias2020generating}. We focus on five types of URLs from the answer context: \emph{arxiv.org}, \emph{dl.acm.org}, \emph{doi.org}, \emph{researchgate.net}, \emph{www.nature.com}, which can indicate publications cited by users. We extract these URLs by regular expression patterns and retrieve paper titles by parsing the URLs directly or visiting the HTML resources or APIs through URLs. Then we align the extracted papers with the OAG paper database \cite{zhang2019oag} to retrieve more information of papers, especially abstract. The papers which cannot be found in the database or whose corresponding abstract is missing in the database are discarded. Finally we only keep the question-paper pairs with complete title and abstract text.


\subsubsection{Zhihu}
Zhihu is a Chinese Q\&A forum which contains kinds of scientific questions. Zhihu questions are not clearly divided by several disciplines, but each question is marked by tags. In fact we find that most answers citing papers are mainly related to only a few fields such as computer science, psychology, biology and physics. To construct the question-paper pairs, we extract the English strings in the Chinese-based answer texts, and search the strings in the OAG paper database \cite{zhang2019oag} to judge whether they are paper titles. Then we match the papers to the corresponding questions to form question-paper pairs and 
%Because Zhihu is not a specialized forum for academic topics, there are more questions not suitable for our task than Stack Exchange, suck as asking for study recommendation or discussing about a conference in a special year. Thus we both using keyword matching and manually checking to delete them from the dataset. 
}












\section{Experiment}
We present extensive experiments over in-domain OpenQA datasets following DPR~\cite{karpukhin2020dense}, together with cross-domain and cross-topic generalization benchmarks BEIR~\cite{thakur2021beir} and OAG-QA. Our surprising findings are summarized as follows:

\begin{itemize}[leftmargin=*,itemsep=0pt,parsep=0.1em,topsep=0.1em,partopsep=0.1em]
    \item \textbf{In-domain Parameter-efficiency:} with less than 0.1\% tuned parameters, parameter-efficient P-Tuning v2 and BitFit can be comparable to full-parameter fine-tuned retrievers, drastically cutting down necessary task-specific storage and memory.
    \item \textbf{Cross-domain \& Cross-topic Generalization:} With similar in-domain performance, parameter-efficient P-Tuning v2 can substantially improve neural retrievers' generalization across domains and topics, as is demonstrated on both BEIR and OAG-QA benchmarks.
\end{itemize}

\subsection{In-domain Parameter-efficiency}
In this section, we describe the data and settings we used for the in-domain OpenQA experiments and evaluate the retrieval performance of the parameter efficient methods.
\subsubsection{Question Answering Datasets.}
We follow \cite{karpukhin2020dense} to use five open-QA datasets and their train/test/valid splits: Natural Questions (NQ)~\cite{kwiatkowski2019natural}, TriviaQA~\cite{joshi2017triviaqa}, WebQuestions (WQ)~\cite{berant2013semantic}, CuratedTREC (TREC)~\cite{baudivs2015modeling} and SQuAD v1.1~\cite{rajpurkar2016squad}. We follow \cite{karpukhin2020dense} to use the split text blocks from the English Wikipedia dump as the retrieval candidate set, which contains 21,015,324 passages.

\subsubsection{Settings.}
We evaluate the in-domain performance using the Dense Passage Retrieval (DPR) Model proposed by \cite{karpukhin2020dense}. We train our DPR model with four different parameter-efficient techniques: Adapters~\cite{houlsby2019parameter}, \pt~\cite{liu2021gpt}, P-Tuning v2~\cite{liu2021p} and BitFit~\cite{zaken2021bitfit}, which are introduced in Section~\ref{sec:4.2}, and compare them against the original full-model fine-tuned DPR baseline. Following \cite{karpukhin2020dense}, we evaluate our model on multi-dataset setting where the training data is combining from all datasets excluding SQuAD and evaluation is conducted on each dataset separately.

We use top-$k$ retrieval accuracy as our evaluation metric, which measures the percentage of questions that have at least one document containing the answer in the top $k$ retrieved documents. In our experiments, we report the results on both top-20 and top-100 accuracy.

\subsubsection{Results.}
\hide{We compare four state-of-the-art parameter efficient methods with conventional fine-tuning in DPR model over the five openQA datasets, using the top-20 and top-100 accuracy.} We identify the best-performed hyper-parameters for each method and the results are shown in Table \ref{tab:openqa}. P-Tuning v2 and BitFit are comparable to fine-tuned baseline on all datasets as expected. P-Tuning v2 is able to outperform consistently the baseline. Moreover, P-Tuning v2 performs the best on all datasets except for SQuAD. We speculate that the reason lies in the difference of SQuAD from the other four datasets, where data was collected from only 500+ Wikipedia articles, and thus the distribution of training examples is extremely biased. On the other hand, \pt performs a bit weaker than the fine-tuned baseline and Adapter shows very poor performance. 

The results empirically demonstrate that using suitable parameter-efficient methods can significantly cut down necessary parameters to 0.1\% and provide competitive performance in in-domain data. According to the average scores of four parameter-efficient methods, we select P-Tuning v2 with the highest accuracy for later zero-shot generalization experiments.


\subsection{Cross-domain Generalization}
To examine the zero-shot generalization of parameter-efficient techniques thoroughly, we introduce our cross-domain experiments below.
% both cross-domain and cross-topic analysis. Below we first introduce the benchmark and settings for cross-domain experiments.

\subsubsection{Benchmark.}
We adopt Benchmarking-IR(BEIR)~\cite{thakur2021beir}, a one-stop zero-shot evaluation benchmark for diverse retrieval tasks, for comparison and evaluation of model generalization. BEIR consists of 18 English zero-shot evaluation datasets (15 of them are available) from 9 heterogeneous retrieval tasks where lengths of queries and documents differ, and 9 domains. The datasets vary from corpus sizes (3.6k - 15M documents) and text types (news articles vs. scientific papers) as well.

\subsubsection{Settings.}\label{sec:cross-domain}
Following \cite{thakur2021beir}, we trained the models on one dataset and report the zero-shot performances on the other datasets. We choose DPR~\cite{karpukhin2020dense} from dense retrieval approaches and ColBERT~\cite{khattab2020colbert} from late-interaction retrieval approaches to explore the retrieval effectiveness under parameter-efficient and full-model settings. We select P-Tuning v2~\cite{liu2021p} as the parameter-efficient technique to be examined and compare it with the original full-training model. Following the settings of BEIR, we use the open-sourced Multi-dataset DPR model and ColBERT model trained on MS MARCO~\cite{nguyen2016ms}.

% For DPR~\cite{karpukhin2020dense}, we follows \cite{thakur2021beir} to use the open-sourced Multi model performs instead of single NQ~\cite{kwiatkowski2019natural} model, and for ColBERT~\cite{khattab2020colbert}, we reproduce a bert-base model using MS MARCO~\cite{nguyen2016ms} dataset.

To obtain comparable evaluation across datasets and tasks in BEIR~\cite{thakur2021beir}, we use Normalized Cumulative Discount Gain (nDCG@k) to involve both binary and graded relevance measures for ranking quality. 

\subsubsection{Results.}
Table \ref{tab:beir} reports the results of DPR and ColBERT on the 15 datasets of BEIR. We compare the models trained by parameter-efficient P-Tuning v2 against the models trained by full-model fine-tuning as baselines using nDCG@10. 

For DPR, P-Tuning v2 generalizes better than the baseline model on all datasets except for MS MARCO and DBPedia. We observe that the datasets where our method improves by more than 5 points, such as Touche-2020 and SciFact, usually consist of long documents with average lengths over 200. We conjecture that it benefits from more information on longer documents. In summary, P-Tuning v2 achieves a 5.2\% improvement on the fine-tuned baseline on the average score over all datasets (except MS MARCO). Thus, P-Tuning v2 greatly improves the out-of-domain generalization of dense retrieval models.

On the other hand, ColBERT trained by P-Tuning v2 is able to perform better than the fine-tuned ColBERT on almost all (13/15) datasets. P-Tuning v2 slightly underperforms on NQ and Quora where documents are relatively short. For the out-of-domain average scores, P-Tuning v2 outperforms the baseline ColBERT by 2.4\%. Compared to dense retrieval approaches, it appears that late-interaction helps improve out-of-distribution generalization but P-Tuning v2 still gains an advancement on generalization. In conclusion, the results demonstrate that with similar in-domain performance, P-Tuning v2 can improve zero-shot generalization on out-of-domain data by a large margin compared to conventional fine-tuning.

\begin{table}[t]
    \centering
    \caption{Zero-shot cross-domain generalization, zero-shot evaluated on 15 datasets of BEIR~\cite{thakur2021beir}.  \textmd{All scores denote \textbf{nDCG@10}. (``*'' indicates the in-domain performances; ``FT'' refers to fine-tuning; ``PT2'' refers to P-Tuning v2)}}
    \footnotesize
    \renewcommand\arraystretch{1.1}
    \renewcommand\tabcolsep{1.8pt}
    \input{tables/beir}
    \label{tab:beir}
\end{table}


\subsection{Cross-topic Generalization}
In addition to cross-domain generalization, cross-topic generalization is a more pragmatic and meaningful challenge for retrieval tasks. Here we explore the cross-topic performance of different training methods.

\begin{table}[t]
    \centering
    \caption{Zero-shot cross-topic generalization, zero-shot evaluated on 22 disciplines of OAG-QA.  \textmd{All scores denote \textbf{Top-20}. (``FT'' refers to fine-tuning; ``PT2'' refers to P-Tuning v2)}}
    \footnotesize
    \renewcommand\arraystretch{1.05}
    \renewcommand\tabcolsep{2.5pt}
    \input{tables/oagqa-results}
    \label{tab:oagqa}
\end{table}

\subsubsection{Benchmark.}
To verify the effectiveness of cross-topic generalization, we use a self-constructed zero-shot evaluation benchmark OAG-QA.\hide{, which is a collection of 17,948 unique queries from 22 scientific disciplines and 87 fine-grained topics. constructed from two influential Question-and-Answer websites: Stack Exchange and Zhihu. OAG-QA has a two-level hierarchical structure where each topic is under a specific discipline.} More details of OAG-QA are described in \ref{tab:oagqa-stats}. Given each topic, we sample 10,000 candidate papers including the groundtruth and take their titles and abstracts as the corpus.  

\subsubsection{Settings.}
We use the same trained DPR~\cite{karpukhin2020dense} and ColBERT~\cite{khattab2020colbert} model introduced in \ref{sec:cross-domain} and conduct a zero-shot evaluation. We measure top-$20$ retrieval accuracy on the dataset of each topic and report the average scores over each discipline.



\subsubsection{Results.}
Table \ref{tab:oagqa} compares models trained by P-Tuning v2 and fine-tuned model as baseline using top-20 retrieval accuracy. P-Tuning v2 outperforms fine-tuning in 20/22 topics in DPR and 18/22 topics in ColBERT respectively. Specifically, P-Tuning v2 performs poorly in Algebra and Linear algebra, two fields which contain a large number of mathematical symbols, in both DPR and ColBERT at the same time. \hide{On the other hand, DPR with P-Tuning v2 outperforms the baseline by about 5\% in Artificial neural network, Computer vision, and Machine learning, which are the topics in Computer Science.}

% Although ColBERT with P-Tuning v2 has two weaker performances, they are only 0.4 points worse, which is still comparable. Similar to DPR, ColBERT trained by P-Tuning v2 also generalizes well in topics of Computer Science, such as Algorithm, Natural language processing, and Machine learning, where P-Tuning v2 improves by about 3\%.

Overall, the average scores over 22 domains of P-tuning are better than that of baseline. P-Tuning v2 gains 2.6\% and 1.2\% improvement for DPR and ColBERT respectively.

% \subsection{Number of Trainable Parameters}\label{sec:param}

% As shown in Table~\ref{tab:openqa} and Table~\ref{tab:beir}, P-Tuning v2 matches or exceeds the fine-tuning baseline on both in-domain and out-of-domain datasets. We explore the relationship between the number of trainable parameters and the model performance on in-domain dataset NQ and out-of-domain dataset SciFact using DPR model (Cf. Figure~\ref{fig:param}). As shown in Figure\ref{fig:param}, not all methods benefit monotonically from having more trainable parameters. We find that P-Tuning v2 with more parameters does perform better than \pt and BitFit but Adapter, which contains comparable parameters to P-Tuning v2, shows poor performance. 

% \begin{figure}[ht]
%   \centering
%   \begin{subfigure}
%      \centering
%      \includegraphics[width=0.85\linewidth]{figures/exp_nq.png}
%   \end{subfigure}
%   \begin{subfigure}
%      \centering
%      \includegraphics[width=0.85\linewidth]{figures/exp_scifact.png}
%   \end{subfigure}
  
% %   \includegraphics[width=0.95\linewidth]{figures/param.png}
%   \caption{Retrieval performance vs. number of trainable parameters of four parameter-efficient methods on in-domain dataset NQ and out-of-domain dataset SciFact. \textmd{P-Tuning v2 shows better scalability and task performance.}}
%   \label{fig:param}
% \end{figure}

% We also observe that the generalization performance drops on SciFact when we use a longer prefix in P-Tuning v2. The in-domain performance on NQ is relatively stable when we use different lengths of the prefix in P-Tuning v2. We conjecture that a shorter prefix with fewer parameters benefits out-of-domain distribution. The specific numbers of parameters and experiment scores are listed in Table~\ref{tab:param-dpr}. In addition to DPR, we also conduct a similar comparison for ColBERT, which is described in Table~\ref{tab:param-colbert}.


==> C_PE_methods.tex <==
\vpara{Adapters~\cite{houlsby2019parameter,pfeiffer2020AdapterHub}.}
% \hide{Adapter module is an alternative to fine-tuning when transferring pre-trained language models to downstream tasks.} 
The adapter approach inserts small modules between transformer layers. 
To limit the number of parameters, the small modules take the shape of a bottleneck. 
The input of the adapter layer $h$ is first projected to a vector of lower dimension $r$ with $W_\text{down} \in \mathrm{R}^{d\times r}$. 
An activation function $f(\cdot)$ is followed and then an up-projection $W_{up} \in \mathrm{R}^{r\times d}$ projects the output back to its original dimension. 
They are surrounded by a residual connection, leading to a form of:
\begin{equation}
    h \leftarrow h + f(hW_\text{down})W_{up}
\end{equation}
Adapters have been shown effective on various tasks including natural language understanding \cite{houlsby2019parameter} and question answering~\cite{Pfeiffer2021AdapterFusionNT}.

\vpara{\pt~\cite{liu2021gpt}.}
Template input with handcrafted prompt has been used to transfer the pre-trained knowledge to downstream tasks. 
Given a language model, a sequence of discrete input tokens $x_{0:n}=\{x_0,x_1...x_n\}$ are mapped to input embeddings $\{e(x_0)...e(x_n)\}$ by the embedding layer. 
% \hide{Given the embedding generated by the language model, a set of target tokens $y$ are used for downstream tasks.} 
The function of the prompt $p$ is to organize the context $x$, the target $y$ into a template T. 
However, discrete handcraft prompts suffer from arduous searching and volatile performance, and thus continuous prompts are proposed. 
For example, given the template $T = \{[P_{0:i}], x, [P_{i+1:m}], y\}$, model's inputs are:
\begin{equation}
    \{h_0, h_1,...h_i,e(x),h_{i+1},...,h_m,e(y)\}
\end{equation}
where the $h_i$ are the trainable.
The continuous prompts can thus be differentially optimized.
% \hide{Prompt-tuning empirically proved to be effective on various downstream tasks like natural language understanding.}

\vpara{Prefix-tuning~\cite{li2021prefix} \& P-tuning v2~\cite{liu2021p}.}
Please refer to Section \ref{sec:4.2}.
% Prefix-tuning is approached by concatenating $l$ trainable prefix vectors to the keys and values of the attention on each layer of the language models. Specifically, given the original key vectors $K \in \mathrm{R}^{l \times d}$ and value vectors $V \in \mathrm{R}^{l \times d}$, trainable vectors $P_k, P_v$ are correspondingly concatenated to $K$ and $V$. The computation of an attention head becomes:
% \begin{equation}
% \small
%     head_i(x) = \mathrm{Attention}(xW^{(i)}, [P^{(i)}_k:K^{(i)}], [P^{(i)}_v:V^{(i)}])
% \end{equation}
% Here the superscript $(i)$ refers to the part of the vectors that correspond to the i-th head.
% It has been empirically proved comparable to fine-tuning on a wide range of downstream tasks, including text generation~\cite{li2021prefix}, natural language understanding (NLU) and sequence labeling~\cite{liu2021p}. In this work, since retrieval is more related to NLU, we employ P-tuning v2's implementation, which makes several crucial optimizations on top of prefix-tuning to ensure its performance.


\vpara{BitFit~\cite{zaken2021bitfit}.}
Bit-fit refers to only tuning the bias term of the entire pre-trained language models. Specifically, each layer of BERT consists of self-attention, FFN and LayerNorm operations. 
The self-attention layers are in the form of equation~\ref{eq:attention}.
The FFN take the form of:
\begin{equation}
    FFN(x) = \max (W_mx + b_m, 0)
\end{equation}
And the LayerNorm has the expression:
\begin{equation}
    LN(x) = g\cdot\frac{x-\mu}{\sigma} + b_{ln}
\end{equation}

The collection of all bias $b(\cdot)$ are the only trainable parameters in the network.

==> tables/oagqa.tex <==

\begin{longtable}{llllll}
\small
\caption{OAG-QA Statistics} \\
\toprule
Discipline                                  & Topic                              & \#Query & Train & Test & \#Query               \\
\midrule
\endfirsthead
\caption[]{OAG-QA Statistics（continued）} \\
\toprule
Discipline                                  & Topic                              & \#Query & Train & Test & \#Query               \\
\midrule
\endhead
\bottomrule
\endfoot
\multirow{7}{*}{\textbf{Geometry}}           & geometry                        & 230      & 20    & 210   & \multirow{7}{*}{1380}  \\
       & algebraic geometry             & 188      & 20    & 168   &                        \\
                                    & algebraic topology             & 131      & 20    & 111   &                        \\
                                    & differential geometry          & 230      & 20    & 210   &                        \\
                                    & group theory                   & 248      & 20    & 228   &                        \\
                                    & category                        & 191      & 20    & 171   &                        \\
                                    & topology                        & 162      & 20    & 142   &                        \\
\midrule
\multirow{3}{*}{\textbf{Statistics}}         & mathematical statistics        & 144      & 20    & 124   & \multirow{3}{*}{516}   \\
                                    & bayes theorem                  & 134      & 20    & 114   &                        \\
                                    & probability theory             & 238      & 20    & 218   &                        \\
\midrule
\multirow{2}{*}{\textbf{Algebra}}            & algebra                         & 280      & 20    & 260   & \multirow{2}{*}{387}   \\
                                    & polynomial                      & 107      & 20    & 87    &                        \\
\midrule
\multirow{5}{*}{\textbf{Calculus}}           & calculus                        & 242      & 20    & 222   & \multirow{5}{*}{868}   \\
                                    & partial differential equation & 200      & 20    & 180   &                        \\
                                    & functional analysis            & 127      & 20    & 107   &                        \\
                                    & hilbert space                  & 127      & 20    & 107   &                        \\
                                    & real analysis                  & 172      & 20    & 152   &                        \\
\midrule
\multirow{4}{*}{\textbf{Number theory}}      & number theory                  & 274      & 20    & 254   & \multirow{4}{*}{899}   \\
                                    & combinatorics                   & 221      & 20    & 201   &                        \\
                                    & set theory                     & 179      & 20    & 159   &                        \\
                                    & prime number                   & 225      & 20    & 205   &                        \\
\midrule
\multirow{2}{*}{\textbf{Linear Algebra}}     & linear algebra                 & 220      & 20    & 200   & \multirow{2}{*}{350}   \\
                                    & matrix                          & 130      & 20    & 110   &                        \\
\midrule
% \multirow{11}{*}{\textbf{Astrophysics}}      & astronomy                       & 108      & 20    & 88    & \multirow{11}{*}{1575} \\
%                                     & astrophysics                    & 101      & 20    & 81    &                        \\
%                                     & universe                        & 112      & 20    & 92    &                        \\
%                                     & cosmology                       & 159      & 20    & 139   &                        \\
%                                     & general relativity             & 191      & 20    & 171   &                        \\
%                                     & special relativity             & 132      & 20    & 112   &                        \\
%                                     & spacetime                       & 172      & 20    & 152   &                        \\
%                                     & dark matter                    & 176      & 20    & 156   &                        \\
%                                     & black hole                     & 160      & 20    & 140   &                        \\
%                                     & entropy                         & 127      & 20    & 107   &                        \\
%                                     & string theory                  & 137      & 20    & 117   &                        \\
% \midrule
% \multirow{12}{*}{\textbf{Quantum Mechanics}} & quantum mechanics              & 467      & 20    & 447   & \multirow{12}{*}{2385} \\
%                                     & quantum entanglement           & 101      & 20    & 81    &                        \\
%                                     & quantum field theory          & 295      & 20    & 275   &                        \\
%                                     & quantum gravity                & 154      & 20    & 134   &                        \\
%                                     & quantum information            & 190      & 20    & 170   &                        \\
%                                     & particle physics               & 247      & 20    & 227   &                        \\
%                                     & photon                          & 125      & 20    & 105   &                        \\
%                                     & supersymmetry                   & 245      & 20    & 225   &                        \\
%                                     & thermodynamics                  & 213      & 20    & 193   &                        \\
%                                     & experimental physics           & 143      & 20    & 123   &                        \\
%                                     & conformal field theory        & 101      & 20    & 81    &                        \\
%                                     & gauge theory                   & 104      & 20    & 84    &                        \\
% \midrule
% \multirow{5}{*}{\textbf{Physics}}            & classical mechanics            & 115      & 20    & 95    & \multirow{5}{*}{862}   \\
%                                     & condensed matter physics      & 201      & 20    & 181   &                        \\
%                                     & optics                          & 151      & 20    & 131   &                        \\
%                                     & electromagnetism                & 224      & 20    & 204   &                        \\
%                                     & mathematical physics           & 171      & 20    & 151   &                        \\
% \midrule
% \multirow{4}{*}{\textbf{Chemistry}}          & organic chemistry              & 332      & 20    & 312   & \multirow{4}{*}{1082}  \\
%                                     & chemical synthesis             & 240      & 20    & 220   &                        \\
%                                     & inorganic chemistry            & 218      & 20    & 198   &                        \\
%                                     & physical chemistry             & 190      & 20    & 170   &                        \\
%                                     & computational chemistry        & 102      & 20    & 82    &                        \\
% \midrule
% \multirow{2}{*}{\textbf{Biochemistry}}       & biochemistry                    & 129      & 20    & 109   & \multirow{2}{*}{442}   \\
%                                     & cell biology                   & 313      & 20    & 293   &                        \\
% \midrule
% \multirow{3}{*}{\textbf{Health Care}}        & health care                    & 288      & 20    & 268   & \multirow{3}{*}{623}   \\
%                                     & endocrinology                   & 111      & 20    & 91    &                        \\
%                                     & physiology                      & 224      & 20    & 204   &                        \\
% \midrule
% \multirow{2}{*}{\textbf{Natural Science}}    & natural science                & 193      & 20    & 173   & \multirow{2}{*}{664}   \\
%                                     & evolutionary biology           & 471      & 20    & 451   &                        \\
% \midrule
% \multirow{2}{*}{\textbf{Psychology}}          & social psychology              & 223      & 20    & 203   & \multirow{2}{*}{571}   \\
%                                     & cognitive neuroscience         & 348      & 20    & 328   &                        \\
% \midrule
% \multirow{2}{*}{\textbf{Algorithm}}          & algorithm                       & 386      & 20    & 366   & \multirow{2}{*}{575}   \\
%                                     & graph theory                   & 189      & 20    & 169   &                        \\
% \midrule
% \multirow{2}{*}{\textbf{Neural Network}}     & artificial neural network     & 488      & 20    & 468   & \multirow{2}{*}{590}   \\
%                                     & cognitive science              & 102      & 20    & 82    &                        \\
% \midrule
% \multirow{3}{*}{\textbf{Computer Vision}}    & computer vision                & 315      & 20    & 295   & \multirow{3}{*}{661}   \\
%                                     & computer graphics images      & 68       & 20    & 48    &                        \\
%                                     & convolutional neural network  & 278      & 20    & 258   &                        \\
% \midrule
% \multirow{5}{*}{\textbf{Data Mining}}        & data mining                    & 131      & 20    & 111   & \multirow{5}{*}{694}   \\
%                                     & feature selection              & 130      & 20    & 110   &                        \\
%                                     & cross validation               & 117      & 20    & 97    &                        \\
%                                     & time series                    & 224      & 20    & 204   &                        \\
%                                     & cluster analysis               & 92       & 20    & 72    &                        \\
% \midrule
\multirow{3}{*}{\textbf{Deep Learning}}      & deep learning                  & 372      & 20    & 352   & \multirow{3}{*}{791}   \\
                                    & optimization algorithm         & 238      & 20    & 218   &                        \\
                                    & reinforcement learning         & 181      & 20    & 161   &                        \\
\midrule
\multirow{1}{*}{\textbf{Machine Learning}}   & machine learning               & 583      & 20    & 563   & \multirow{1}{*}{1208}  \\
                                    & hidden markov model           & 112      & 20    & 92    &                        \\
                                    & classifier                      & 269      & 20    & 249   &                        \\
                                    & linear regression              & 244      & 20    & 224   &                        \\
\midrule
\multirow{2}{*}{\textbf{NLP}}                & natural language processing   & 305      & 20    & 285   & \multirow{2}{*}{587}   \\
                                    & recurrent neural network      & 282      & 20    & 262   &                        \\
\midrule
\textbf{Economics}                           & economics                       & 238      & 20    & 218   & 238                    \\
\midrule
\textbf{总数}                                  & -                               & 17948    & 1740  & 16208 & 17948                  
\label{tab:oagqa-stats}
\end{longtable}
